Tight Query Complexity Lower Bounds for PCA via Finite Sample Deformed Wigner Law

We prove a \emph{query complexity} lower bound for approximating the top $r$ dimensional eigenspace of a matrix. We consider an oracle model where, given a symmetric matrix $\mathbf{M} \in \mathbb{R}^{d \times d}$, an algorithm $\mathsf{Alg}$ is allowed to make $\mathsf{T}$ exact queries of the form $\mathsf{w}^{(i)} = \mathbf{M} \mathsf{v}^{(i)}$ for $i$ in $\{1,...,\mathsf{T}\}$, where $\mathsf{v}^{(i)}$ is drawn from a distribution which depends arbitrarily on the past queries and measurements $\{\mathsf{v}^{(j)},\mathsf{w}^{(i)}\}_{1 \le j \le i-1}$. We show that for every $\mathtt{gap} \in (0,1/2]$, there exists a distribution over matrices $\mathbf{M}$ for which 1) $\mathrm{gap}_r(\mathbf{M}) = \Omega(\mathtt{gap})$ (where $\mathrm{gap}_r(\mathbf{M})$ is the normalized gap between the $r$ and $r+1$-st largest-magnitude eigenvector of $\mathbf{M}$), and 2) any algorithm $\mathsf{Alg}$ which takes fewer than $\mathrm{const} \times \frac{r \log d}{\sqrt{\mathtt{gap}}}$ queries fails (with overwhelming probability) to identity a matrix $\widehat{\mathsf{V}} \in \mathbb{R}^{d \times r}$ with orthonormal columns for which $\langle \widehat{\mathsf{V}}, \mathbf{M} \widehat{\mathsf{V}}\rangle \ge (1 - \mathrm{const} \times \mathtt{gap})\sum_{i=1}^r \lambda_i(\mathbf{M})$. Our bound requires only that $d$ is a small polynomial in $1/\mathtt{gap}$ and $r$, and matches the upper bounds of Musco and Musco '15. Moreover, it establishes a strict separation between convex optimization and \emph{randomized}, "strict-saddle" non-convex optimization of which PCA is a canonical example: in the former, first-order methods can have dimension-free iteration complexity, whereas in PCA, the iteration complexity of gradient-based methods must necessarily grow with the dimension.

==> concentration.tex <==
%!TEX root = main.tex
\section{Concentration of Measure}


\section{}


==> lin_alg.tex <==
%!TEX root = main.tex

\section{A Recursion for Rank-One}

Let $M = W + \lambda UU^{\top}$, where $U \in \calO(d,k)$. For all $\theta \in \col(U)$, let $M_{\theta} = W + \lambda \theta \theta^{\top}$. 




\begin{lem} Let $v$ be any eigenvector of $M$. Then, $v$ is an eigenvector of $M_{\theta}$ where $\theta = UU^\top v$. 
\end{lem}
\begin{proof}
Let $\theta = UU^{\top} v $. Since $U$ is orthonormal, we name $UU^{\top}v = \theta \theta^{\top} v$, and thus $Mv = Wv + UU^\top v = Wv + \theta \theta^\top v = M_{\theta} v$, so $v$ is an eigenvector of $\theta$.
\end{proof}

\begin{lem}
Suppose that $W \succeq 0$. For either $F(A,v) := v^\top A v$ or $F(A,v) := \|Av\|_2$, we have that 
\begin{eqnarray}
\{v_{\max}(M)\} = \arg\max_{v \in \calS^{d-1}} \sup_{\theta \in U} F(M_{\theta},v) = v_{\max}(\arg\max_{\theta \in U}\lambda_{\max}(M_{\theta}))
\end{eqnarray}
where the $\arg\max$ on the left hand side is unique. Observe that the 
\end{lem}
\begin{proof}
It is straightforward that $\arg\max_{v \in \calS^{d-1}} \sup_{\theta \in U} F(M_{\theta},v) = v_{\max}(\arg\max_{\theta \in U}\lambda_{\max}(M_{\theta}))$, so it suffices to show that $v_{\max}(M) = \arg\max_{v \in \calS^{d-1}} \sup_{\theta \in U} F(M_{\theta},v)$. We being by establishing that $\max_{v \in \calS^{d-1}} \sup_{\theta \in U} F(M_{\theta},v) \ge \lambda_{\max}(M)$. Indeed, by the previous lemma, there exists a $\theta$ such that $v_{\max}(M)$ is an eigenvalue of $M_{\theta}$, and thus (using that $M \succeq 0$)
\begin{eqnarray}
 \lambda_{\max}(M) = v_{\max}(M)^\top M v_{\max}(M) = v_{\max}(M_{\theta})^\top M v_{\max}(M) \le \max_{v \in \calS^{d-1}} \sup_{\theta \in U} F(M_{\theta},v)
\end{eqnarray}

Now, suppose that $v_0 \in \arg\max_{v \in \calS^{d-1}}  \sup_{\theta} F(M_{\theta},v)$, and let $\theta_0 \in \sup_{\theta \in U} F(M_{\theta},v)$. Then, $v_0 \in \arg\max_{v \in \calS^{d-1}}  F(M_{\theta_0},v)$,  and since $M_{\theta} \succ 0$ is symmetric we have that 
\begin{eqnarray}
F(M_{\theta_0},v_{0}) = \lambda_{\max}(M_{\theta_0}) = v_0^\top M_{\theta_0}v_0 
\end{eqnarray}
By the above, $F(M_{\theta_0},v_{0}) \ge \lambda_{\max}(M_{\theta},v_0)$. On the other hand, $M_{\theta_0} \preceq M$ and so $v_0^\top M_{\theta_0}v_0 \le v_0^{\top} M v_0 \le \lambda_{\max}(M)$. Hence, we conclude that $v_0^\top M v_0 = \lambda_{\max}(M)$, whence by uniquenes of $v_{\max}(M) = v_0$. 
\end{proof}

\begin{lem} Suppose that $\inf_{\theta} \lambda_{\max}(M_{\theta}) \ge $
\end{lem}

	

==> main_body.tex <==
\input{intro.tex}
\input{techniques.tex}
\input{related.tex}
\input{results.tex}
\input{reduction_to_estimation.tex}
%\input{notation.tex}
%\input{wigner_reduction}
% Main File Containing info about the top eigenvalue separation



%%%%%%%%%%%%%% Don't read yet

\input{rank_one.tex}
\input{rank_r.tex}
\input{eig_separation.tex}
%\input{quadratic_redux.tex}



==> notation.tex <==
%!TEX root = main.tex


\section{Notation} \maxs{this is very rough, just enough for you (Ahmed) to follow the sections thus far}



==> quadratic_redux.tex <==
%!TEX root = main.tex

\section{}
	We have that
	\begin{eqnarray}
	B^{-1}\theta &=& (\rho I - W - \lambda \theta \theta^\top)^{-1}\theta \\
	&=&(\rho I - W)^{-1}\theta + \lambda \frac{(\rho I - W)^{-1}\theta \theta^\top (\rho I - W)^{-1}\theta}{1 - \lambda \theta^\top (\rho I - W)^{-1}\theta}\\
	&=& (\rho I - W)^{-1}\theta \cdot \{ 1 +  \frac{\theta^\top (\rho I - W)^{-1}\theta}{(1/\lambda) - \theta^\top (\rho I - W)^{-1}\theta}\} \\
	&=& \frac{ (\rho I - W)^{-1}\theta   }{1 - \lambda \theta^\top (\rho I - W)^{-1}\theta}\} 
	\end{eqnarray}
	Moreover, 
	\begin{eqnarray}
	B^{-1}w = (\rho I - W)^{-1}w + \lambda \frac{(\rho I - W)^{-1}\theta \theta^\top (\rho I - W)^{-1} w}{1 - \lambda \theta^\top (\rho I - W)^{-1}\theta} = (\rho I - W)^{-1}w + lot 
	\end{eqnarray}

	Hence, we have $(\rho I - W)^{-1}w$


	Hence,  if $x = \theta + w$,
	\begin{eqnarray}
	\theta^{\top}B^{-1}x = \lambda \frac{\theta^\top(\rho I - W)^{-1}\theta + w^\top(\rho I - W)^{-1}w  }{1 + \lambda\theta^\top (\rho I - W)^{-1}\theta}\}  = \theta^\top B^{-1} \theta + lot
	\end{eqnarray}
	Next, observe that we have $\theta^{\top} $


	Now if $\widehat{x} = B^{-1}x + \xi_B$, where $\xi_B^\top B \xi_B \le \Delta$, then $\widehat{x} = B^{-1}x + B^{-1/2} \xi$, where $\|\xi\| \le \Delta$. Note then that $\max_{|\|\xi\| \le \Delta\|} \langle \theta, B^{-1/2}\xi\rangle^2 = \Delta^2 \|B^{-1/2}\theta\|^2 = \theta^\top B^{-1}\theta \Delta^2 $. Hence, we have

	\begin{eqnarray}
	\langle \theta, \widehat{x} \rangle = \rangle  B^{-1}x + \xi_B , \theta\rangle  \ge \theta^\top B^{-1} \theta + t\sqrt{\Delta \cdot \theta^\top B^{-1} \theta } + LOT
	\end{eqnarray}
	for $t \in [0,1]$
	Next, we have that 
	\begin{eqnarray}
	\|\widehat{x}\|^2 &=& \|B^{-1}w\|
	\end{eqnarray}



	 Now, given a solver, we have
	\begin{eqnarray}
	\langle \frac{\widehat{x}}{\|\widehat{x}\|},\theta \rangle = \frac{\theta^{\top}B^{-1}x + \langle \theta, B^{1/2} \xi_B \rangle}{\|\theta^{\top}B^{-1}x + \langle \theta, B^{1/2} \xi_B\|}
	\end{eqnarray}



\begin{comment}
\section{}
	Given a matrix $M$, define the associated matrix $B$ via $\lambda_* = \lambda_{1}(M)(1+c_0 \gap(M))$ and $B = \lambda_*I - M$.
	\begin{lem} Let $x$ be a unit vector satisfying $\lambda_1(M) - x^\top M x  = \epsilon \cdot \lambda_1(M) \cdot \gap(M)$, for $\epsilon \le 1/2$. Then, if $\widetilde{x}$ satisfies $G(\widetilde{x}) \le \alpha G(x)$, 
	\begin{eqnarray}
	\lambda_1(M) - \widetilde{x}^\top M \widetilde{x} \le (1 + c_0)(1 + 2\epsilon)\frac{\epsilon}{\alpha^2}
	\end{eqnarray}
	\end{lem}

	\begin{lem} Let $x$ be a unit vector, and suppose that there exists a solve which return an $\widetilde{x}$ such that 
	\begin{eqnarray}
	\|B^{1/2}\widetilde{x} - B^{-1/2}x\| \le \frac{1}{2}\sqrt{\lambda_1(M)  \gap (M)   \min\{c_0 \langle v_1(M), x \rangle^2 ,(1 - \langle v_1(M), x \rangle^2)\}} 
	\end{eqnarray}
	Then, $G(\widetilde{x}) \le 6 G(x)$
	\end{lem}
	\begin{proof}
	Let $x = \sum_{i=1}^n \alpha_i v_i(M)$. Then,  
	\begin{eqnarray}
	G(\widetilde{x}) &\le& G(x) \cdot \frac{ \lambda_2(B^{-1}) + \|\xi\|_B/\sqrt{\sum_{i \ge 2} \alpha_i^2/ \lambda_i(B^{-1})}}{\lambda_1(B^{-1}) - \|\xi\|_B/\sqrt{ \alpha_1^2 / \lambda_1(B^{-1})}}\\
	&\le& G(x) \cdot \frac{ \lambda_2(B^{-1})}{\lambda_1(B^{-1})}  \cdot \frac{ 1 + \|\xi\|_B/\sqrt{\sum_{i \ge 2} \alpha_i^2 \lambda_2(B^{-1})^2/\lambda_i(B)}}{1 - \|\xi\|_B/\sqrt{ \alpha_1^2 \lambda_1(B^{-1})}}\\\\
	&\le& G(x) \cdot \frac{ 1}{c_0}  \cdot \frac{ 1 + \|\xi\|_B/\sqrt{(1-\alpha_1^2)\lambda_1(M)\gap(M)}}{1 - \|\xi\|_B/\sqrt{  \alpha_1^2/\lambda_1(M) c_0\gap(M)}}\\
	\end{eqnarray}
	Hemce, under the state condtion, the above evaluates to at no more than $6/c_0 G(x)$. 
	\end{proof}

	\begin{proof}[First Lemma]
	By Lemma 3 in [], we have that if $\epsilon \le 1/2$,
	\begin{eqnarray}
	G(x)^2 \le (1 + \frac{\lambda_* - \lambda_1(M)}{\lambda_1(M)\cdot \gap(M)})(1 + \frac{2\epsilon \lambda_1(M)}{\lambda_1(M) \cdot \gap(M)})\frac{\epsilon \cdot \lambda_1(M) \cdot \gap(M)}{\lambda_* - \lambda_1(M)} 
	\end{eqnarray}
	Plugging in $\lambda_* - \lambda_1(M) = c_0 \gap(M)$ and simplifying yields
	\begin{eqnarray}
	(x)^2 \le (1 + c_0)(1 + 2\epsilon)\frac{\epsilon}{c_0}
	\end{eqnarray} 
	Moreover, if $v_1 = v_1(M)$, then by the computation in Lemma 3 of [] and Lemma 2 []
	\begin{eqnarray}
	G(\widetilde{x})^2 &=& \frac{\widetilde{x}^\top B \widetilde{x} - (v_1^\top B \widetilde{x})v_1^\top \widetilde{x}}{(v_1^\top B \widetilde{x})v_1^\top \widetilde{x}}\\
	&\overset{\text{ Lemma 2, }}{\ge}& \frac{\widetilde{x}^\top B \widetilde{x} - (v_1^\top B \widetilde{x})v_1^\top \widetilde{x}}{(v_1^\top B \widetilde{x})v_1^\top \widetilde{x}}\\
	&=& \frac{\widetilde{\epsilon} \lambda_1 \gap(M)}{(\lambda_* - \lambda_1) (v_1^\top \widetilde{x})^2}\\
	&=& \frac{\widetilde{\epsilon} \lambda_1 \gap(M)}{(\lambda_* - \lambda_1)} = \frac{\widetilde{\epsilon}}{c_0}
	\end{eqnarray}
	
	Hence, if $G(\widetilde{x}) \le \alpha G(x)$, and $\lambda_1(M) - \widetilde{x}^\top M \widetilde{x}  = \widetilde{\epsilon} \cdot \lambda_1(M) \cdot \gap(M)$, then we have 
	\begin{eqnarray}
	(1 + c_0)(1 + 2\epsilon)\frac{\epsilon}{c_0} \ge G(x)^2 \ge \alpha^2 G(\widetilde{x})^2 \ge \alpha^2 \frac{\widetilde{\epsilon}}{{c_0}}
	\end{eqnarray}
	Hence, if $\epsilon \le 1/2$, then 
	\begin{eqnarray}
	\widetilde{\epsilon} \le (1 + c_0)(1 + 2\epsilon)\frac{\epsilon}{\alpha^2}
	\end{eqnarray}
	\end{proof}
		
\end{comment}






	

==> texting.tex <==
\subsection{Proof of Proposition~\ref{truncChi_detec}}
	For ease of notation, let $\overline{\Prit}_A =  \overline{\Prit}[\cdot;\{A_{\theta}\}]$. Note that $\overline{\Prit} - \overline{\Prit}_A  \ge 0$, which impies that
	\begin{eqnarray}
	\int |\rmd\overline{\Prit} - \rmd\overline{\Prit}_A| = \int \rmd\overline{\Prit} - \rmd\overline{\Prit}_A = 1 - \overline{\Prit}_A(\calX) := 1-p,
	\end{eqnarray}
	so by the triangle inequality
	\begin{eqnarray*}
	&& \|\Qit - \overline{\Prit}\|_{TV} =\frac{1}{2}\int |\rmd\Qit(x) - \rmd\overline{\Prit}(x)|\\
	&\le& \frac{1}{2}\int |\rmd\Qit(x) - \rmd\Prit_A(x)| + \frac{1}{2} \int |\rmd\overline{\Prit} - \rmd\overline{\Prit}_A| = \frac{1}{2}\int |\rmd \Qit(x) - \rmd\Prit_A(x)| + \frac{1-p}{2},
	\end{eqnarray*}
	Next, since $\Qit$ is a probability measure,
	\begin{eqnarray*}
	\int |\rmd\Qit(x) - \rmd\Prit_A(x)| &=& \Exp_{\Qit} |\frac{\rmd\overline{\Prit}_A}{\rmd\Qit} - 1| \le \sqrt{\Exp_{\Qit} |\frac{\rmd\overline{\Prit}_A}{\rmd\Qit} - 1|^2}\\
	&=& \sqrt{\Exp_{\Qit} |\frac{\rmd\overline{\Prit}_A}{\rmd\Qit}|^2  + 1 - 2\overline{\Prit}_{A}(\calX)} = \sqrt{\Exp_{\Qit} |\frac{d\overline{\Pr}_A}{\rmd\Q}|^2  + 1 - 2p}\\
	&=& \sqrt{\Exp_{\Qit} |\frac{\rmd\overline{\Prit}_A}{\rmd\Qit}|^2  - 1 + 2(1-p) } \le  \sqrt{\Exp_{\Qit} |\frac{\rmd\overline{\Prit}_A}{\rmd\Qit}|^2  - 1} + \sqrt{2(1-p)}.
	\end{eqnarray*}
	Putting pieces together yields the proof.


==> wigner_reduction.tex <==
%!TEX root = main.tex



\subsection{Computing the Conditional Likelihoods\label{Likelihood_Comp}}
We begin by introducing some useful simplifications.  In particular, this implies that $\vi$ is a measurable function of $\itZ_{i-1}$


Second, we assume that $\vone,\dots,\vT$ are orthonormal. This is without loss of generality because one can reconstruct the response $\wi$ to a query $\vi$ by simply quering the projection of $\vi$ onto the orthogonal complement of the previous queries $\vone,\dots,\viminus$, and normalizing. 
Finally, we introduce a simplification which will make our queries resemble queries of the form $\wi = \matu \matu^\top \vi + \text{ i.i.d.\ noise}$.

  We show that, with our modified measurements $\wi = \itP_{i-1}\matM\vi$, then the query-observation pairs $(\vi,\wi)$ have Gaussian likelihoods conditional on $\itZ_i$ and $\matu$.
\begin{lem}[Conditional Likelihoods] \label{ConditionalLemma} Under $\Prit_{u}$ ( the joint law of $\matM$ and $\itZ_T$ on $\{\matu = u\}$), we have
\begin{multline}
\itP_{i-1}\matM\vi \big{|} \itZ_{i-1} \sim \mathcal{N}\left(\lambda (u^\top \vi) \itP_{i-1} u,\frac{1}{d}\itSigma_i \right), \quad \text{where} \quad \itSigma_{i} := \itP_{i-1}\left(I_d+ \vi\viT \right)\itP_{i-1}.
\end{multline}
In particular, $\wi$ is conditionally independent of $\wone,\dots,\wiminus$ given $\vone,\dots,\viminus$ and $\matu = u$.
\end{lem}
Lemma~\ref{ConditionalLemma} is proved in Appendix~\ref{CondLemProof}. We remark that $\itSigma_i$ is rank-deficient, with its kernel being equal to the span of $\{\vone,\dots,\viminus\}$. Nevertheless, because the mean vector $\lambda (u^\top \vi) \itP_{i-1} u$ lies in the orthogonal complement of $\ker \itSigma_i$, computing $\itSigma_i^{-1} (\lambda (u^\top \vi) \itP_{i-1} u)$ can be understood as $\itSigma_i^{\dagger} (\lambda (u^\top \vi) \itP_{i-1} u)$, where $\dagger$ denotes the Moore-Penrose pseudo-inverse~\cite{horn2012matrix}. We will use the following equality and inequality frequently and without comment: 
\begin{eqnarray}\label{InverseInequality}
\|\lambda v\|_{\frac{1}{d}\itSigma_i}^2 =d \lambda^2 \|v\|_{\itSigma_i}^2, & \text{and} & \|\itP_{i-1}u\|_{\itSigma_i}^2  \le \|u\|^2. 
\end{eqnarray}
These just follow from the facts that $\itP_{i-1}$ is an orthogonal projection and $\itSigma_i \succeq \itP_{i-1}$, and so $\itP_{i-1}\itSigma_i^{\dagger}\itP_{i-1} \preceq I$. 

